Extensible Pattern Matching in an Extensible Language

Pattern matching is a widely used technique in functional languages, especially those in the ML and Haskell traditions, where it is at the core of the semantics. In languages in the Lisp tradition, in contrast, pattern matching it typically provided by libraries built with macros. We present match, a sophisticated pattern matcher for Racket, implemented as language extension. using macros. The system supports novel and widely-useful pattern-matching forms, and is itself extensible. The extensibility of match is implemented via a general technique for creating extensible language extensions.

==> style.tex <==
% style.tex start


\author{Sam Tobin-Hochstadt}
\institute{PLT @ Northeastern University\\
           {\tt samth@ccs.neu.edu}}

\renewcommand{\sectionNewpage}{}
\newcommand{\titleAndVersion}[2]{\title{#1}\maketitle}

\newcommand\overmath[1]{\ensuremath{\overline{#1}}}

%style.tex end

